On the range of validity of parabolic models for fluid flow through isotropic homogeneous porous media

Lattice-Boltzmann methods are established mesoscopic numerical schemes for fluid flow, that recover the evolution of macroscopic quantities (viz., velocity and pressure fields) evolving under macroscopic target equations. The approximated target equations for fluid flows are typically parabolic and include a (weak) compressibility term. A number of Lattice-Boltzmann models targeting, or making use of, flow through porous media in the representative elementary volume, have been successfully developed. However, apart from two exceptions, the target equations are not reported, or the assumptions for and approximations of these equations are not fully clarified. Within this work, the underlying assumption underpinning parabolic equations for porous flow in the representative elementary volume, are discussed, clarified and listed. It is shown that the commonly-adopted assumption of negligible hydraulic dispersion is not justifiable by clear argument - and in fact, that by not adopting it, one can provide a qualitative and quantitative expression for the effective viscosity in the Brinkman correction of Darcy law. Finally, it is shown that, under certain conditions, it is possible to interpret porous models as Euler-Euler multiphase models wherein one phase is the solid matrix.

==> Makefile <==
# Makefile: Remove all files/patterns listed in .gitignore by default

# The default target is 'clean' so that just running `make` will remove files.
default: clean

.PHONY: clean
clean:
	@echo "Removing files/patterns from .gitignore..."
	@for pattern in $(shell grep -Ev '^(#|$$)' .gitignore); do \
	  rm -rf $$pattern 2>/dev/null || true; \
	done


==> src/highlights.tex <==
\item Research highlight 1
\item Research highlight 2
\item Research highlight 3
